Suturing Tasks Automation Based on Skills Learned From Demonstrations: A Simulation Study

In this work, we develop an open-source surgical simulation environment that includes a realistic model obtained by MRI-scanning a physical phantom, for the purpose of training and evaluating a Learning from Demonstration (LfD) algorithm for autonomous suturing. The LfD algorithm utilizes Dynamic Movement Primitives (DMP) and Locally Weighted Regression (LWR), but focuses on the needle trajectory, rather than the instruments, to obtain better generality with respect to needle grasps. We conduct a user study to collect multiple suturing demonstrations and perform a comprehensive analysis of the ability of the LfD algorithm to generalize from a demonstration at one location in one phantom to different locations in the same phantom and to a different phantom. Our results indicate good generalization, on the order of 91.5%, when learning from more experienced subjects, indicating the need to integrate skill assessment in the future.

==> paper_draft.tex <==
Robotic surgery has revolutionized the field of medical science by providing surgeons with enhanced dexterity, visualization, and precision during minimally invasive procedures. The Da Vinci Surgical System, a widely adopted robotic platform, has transformed surgical interventions, enabling complex procedures with improved patient outcomes. However, despite the remarkable capabilities of robotic systems, certain repetitive tasks, such as suturing, continue to demand significant manual intervention, which can impose cognitive load on surgeons and impact procedural efficiency.

Automating repetitive surgical tasks has emerged as a promising approach to alleviate the cognitive burden on surgeons, allowing them to focus on critical decision-making and enhance patient care. In this regard, automating suturing has gained significant attention, aiming to reduce surgical time, enhance precision, and ensure consistent suture placement, thereby optimizing surgical outcomes.

In this paper, we present a novel method for automatic suturing path planning using the Da Vinci Research Kit (dVRK). Our approach leverages Learning from Demonstration (LfD) and utilizes user study data obtained from expert surgeons to train the dVRK in performing suturing tasks. Notably, the training data for our method is acquired from a customized simulator that integrates seamlessly with the dVRK, allowing for the collection of surgeon input data identical to real clinical scenarios. Furthermore, the trained model can be directly applied to the dVRK, ensuring its practical applicability.

The utilization of LfD in our method offers several advantages. Firstly, by acquiring data from expert surgeons, we capture their tacit knowledge and best practices, enabling the dVRK to mimic the skills and expertise of highly skilled practitioners. This ensures that the automated suturing path planning closely aligns with the strategies employed by experienced surgeons, promoting safe and effective suturing. Secondly, the integration of a customized simulator with the dVRK enables the collection of user data under realistic clinical scenarios, enhancing the authenticity and relevance of the training process. Lastly, by directly applying the trained model to the dVRK, we facilitate seamless translation of the acquired knowledge into practical surgical applications.

Our research aims to address the challenges associated with automated suturing in robotic surgery, providing a robust and efficient solution for suturing path planning. By utilizing LfD and incorporating a customized simulator integrated with dVRK, we present a method that not only captures expert knowledge but also ensures its direct applicability in real-world surgical scenarios.

The structure of this paper is as follows: Section 2 provides an overview of the related work in the field of automated suturing and highlights the significance of LfD. Section 3 details the methodology employed for training the dVRK using user study data acquired from the customized simulator. Section 4 presents the experimental setup, including the simulator integration and data collection process. Section 5 discusses the results obtained and analyzes the performance of the automated suturing path planning. Finally, Section 6 concludes the paper, summarizing the contributions, limitations, and outlining potential avenues for future research.
